Cost- and QoS-Efficient Serverless Cloud Computing

Cloud-based serverless computing systems, either public or privately provisioned, aim to provide the illusion of infinite resources and abstract users from details of the allocation decisions. With the goal of providing a low cost and a high QoS, the serverless computing paradigm offers opportunities that can be harnessed to attain the goals. Specifically, our strategy in this dissertation is to avoid redundant computing, in cases where independent task requests are similar to each other and for tasks that are pointless to process. We explore two main approaches to (A) reuse part of computation needed to process the services and (B) proactively pruning tasks with a low chance of success to improve the overall QoS of the system. For the first approach, we propose a mechanism to identify various types of "mergeable" tasks, which can benefit from computational reuse if they are executed together as a group. To evaluate the task merging configurations extensively, we quantify the resource-saving magnitude and then leveraging the experimental data to create a resource-saving predictor. We investigate multiple tasks merging approaches that suit different workload scenarios to determine when it is appropriate to aggregate tasks and how to allocate them so that the QoS of other tasks is minimally affected. For the second approach, we developed the mechanisms to skip tasks whose chance of completing on time is not worth pursuing by drop or defer them. We determined the minimum chance of success thresholds for tasks to pass to get scheduled and executed. We dynamically adjust such thresholds based on multiple characteristics of the arriving workload and the system's conditions. We employed approximate computing to reduce the pruning mechanism's computational overheads and ensure that the mechanism can be used practically.

==> B-acknowledgement.tex <==
~
            I sincerely thank my supervisor, Professor \Supervisor, for his constant encouragement and passion for computer science and, especially, for his guidance and support. Thanks to my dissertation committee, Nian-Feng Tzeng, Sheng Chen, and Miao Jin. Thanks to Jame S Gentry, Vaughan Veillion, Ali Mokhtari, Davood Ghatreh Samani, and Shangrui Wu for their assistance in the work of this dissertation. Finally, thanks goes to the Center for Advanced Computer Studies and the Graduate School at the University of Louisiana at Lafayette for their support and guidance.


==> B-dedicatory.tex <==
\vspace*{\fill}
\begin{center}
\textit{
To my parents, Niwet Denninnart and Chareeya Denninnart, my Sister Nicha Denninnart and to all my friends and loved ones.
}
\end{center}
\vspace*{\fill}



==> archiveC2--excludedBG.tex <==
%maybe dedicated page for background?

%\section{Cloud Computing Service}


%BG STYLE, everything moved to RW page, This page is not included

\section{Serverless Cloud Computing (Function as a Service)}
In Serverless computing paradigm, a serverless application usually provided as one or more stateless standalone application code dedicated to handle specific type of request~\cite{peekserverless}. 
In such platform, system provider manage all execution environment such as resource allocating, scaling, scheduling and ensuring availability. To use serverless computing, the end user upload Serverless functions to the handle service request that can be triggered by timer or by event (such as HTTP request). 

In the back end, while the platform usually keep frequently used functions in the memory to enable warm start of the function when a service request arrives. Such treatment is not affordable for infrequently used functions. As such, infrequently used functions are removed from the memory and have to start from cold state for each incoming request. % and then go back to sleep when not required. 
Each of the Service request is submitted into a shared scheduling queue to get executed. This improve cost effectiveness over traditional IaaS model by reducing idle resources wastage (idle time on active machines and also number of pre-warm spare machines.) %for both provider and the user than
Such back-end managements are abstracted from serverless computing user. 

In recent years, most serverless functions are provided as a docker/container style either on top of a dedicated virtual machine or in a shared execution queue. In this study, to maximize the potential benefit provided by serverless computing system, the serverless functions are viewed as stand-alone functional codes or executable objects with some metadata. All service requests are scheduled on a shared scheduling queue and the actual code execution is performed on shared computing resources.

\section{Heterogeneous Computing}
A Heterogeneous Computing (HC) system can be described by two types of heterogeneity: inconsistent and consistent~\cite{ali2000,li2018cost}. Inconsistent machine heterogeneity refers to differences in machine architecture (\eg CPU versus GPU versus FPGA~\cite{zahaf2017het, zhao2017fpga,hong2017gpu}). Consistent machine heterogeneity describes the differences among machines of a certain architecture (\eg different clock speeds). Compute services offered by cloud providers are a good example of an HC system. Amazon cloud~\cite{aws} offers inconsistent heterogeneity in form of various Virtual Machine (VM) types, such as CPU-Optimized, Memory-Optimized, Disk-Optimized, and Accelerated Computing (GPU and FPGA). Within each type, various VMs are offered with consistent performance scaling with price~\cite{aws}. Moreover, both consistent and inconsistent heterogeneity can exist in arriving tasks. For example, an HC system dedicated to processing live video streams is responsible for many categorically different types of tasks: changing video stream resolution, changing the compression standard, changing video bit-rate~\cite{li2018cost}. Each of these task types can be consistently heterogeneous within itself (\eg it takes longer to change resolution of 10 seconds of video, compared to 5). 


Many HC systems (\eg~\cite{zong2017marcher,LONI}) present both consistent and inconsistent heterogeneity in machines used and task types processed~\cite{smith09}. These systems present cases where each task type can execute differently on each machine type, where machine type $A$ performs task type 1 faster than machine type $B$ does, but is slower than other machine types for task type 2. Specifically, compute intensive tasks run faster on (\ie matches better with) a GPU machine whereas tasks with memory and disk accesses bottlenecks (\eg in-memory databases~\cite{wang2014using,dos2015smart,malensek2016minerva}) runs faster on a CPU-based machine. 

All of this heterogeneity results in uncertainty for a given task's execution time, thus, inefficiency of resource allocation~\cite{ali2000}. Accordingly, a major challenge in HC systems is to assign tasks to machines to optimize performance goal of the system~\cite{ali2000}.

\section{Task Request Mapping Heuristics}
\begin{figure}[ht]
  \centering
  \includegraphics[width=0.8\textwidth]{figures/C3/ConventionalMapping.pdf}
  \caption{Overview of mapping heuristics widely-used in various types of distributed systems. \label{fig:convtree} }
\end{figure}

Serverless (and cloud computing system in general) have such a wide variety of performance characteristics and QoS requirement. 
In both homogenerous computing system and heterogeneous computing system, optimal task-machine mapping is proven to be an NP-complete problem \cite{coffman76,Ibarra77}. Therefore, a large body of mapping heuristics (\eg~\cite{Braun01,Ibarra77,madni2017performance}) have been developed for these systems. Figure~\ref{fig:convtree} provides an overview of mapping heuristics commonly used in heterogeneous and homogeneous systems. In particular, mapping heuristics of HC systems can be further categorized based on those operate in immediate-mode and in batch-mode resource allocation systems. 


Immediate-mode mapping heuristics do not hold tasks in an arrival queue and they are simpler to develop. In batch-mode heuristics, however, mapping occurs both upon task arrival (when machine queues are not full) and upon task completion. 
Batch-mode heuristics generally use an auxiliary structure, known as \emph{virtual queue}, where arriving tasks are examined on different machine queues. These heuristics commonly use a two-phase process for decision making. In the first phase, the heuristic finds the best machine for each task, by virtue of a per-heuristic objective. In the second phase, from task-machine pairs obtained in the first phase, the heuristic attempts to choose the best machine-task pairs for each available machine queue slot. After all slots are filled, or when the unmapped queue is emptied, the virtual mappings are pushed (assigned) to the machine queues, and the mapping method is complete.

Although mapping heuristics used in homogeneous computing systems are of batch nature, their logic is simpler than those used in batch-mode of HC systems. Here we review widely-used heuristics in both heterogeneous and homogeneous computing systems.

\subsection{Immediate-Mode Mapping Heuristics for Heterogeneous Computing Systems}
\begin{figure}[ht]
    \centering 
    \includegraphics[width=0.6\textwidth]{figures/C3/mapper_imm.pdf} 
    \label{fig:ImmSchedule}
     \caption{Immediate-mode resource allocation operates immediately, upon arrival of a task to the system.}
\end{figure}

\paragraph{Round Robin (RR)}  %changed from FCFS
In RR~\cite{li2016high}, incoming tasks are assigned in a round robin manner to an available machine, from Machine 0 to Machine $n$.

\paragraph{Minimum Expected Execution Time (MET)} 
In MET, the incoming task $i$ is assigned to the machine that offers the minimum expected execution time (\ie the average of the $PET(i,j)$ for task $i$ on machine $j$). 

%recheck def, if convolve or sum of avg
\paragraph{Minimum Expected Completion Time (MCT)} In MCT, the incoming task is assigned to the machine that offers the minimum expected completion time. The completion time is obtained based on the accumulated expected execution time of tasks queued in a given machine.

\paragraph{K-Percent Best (KPB)} 
KPB is a combination of MCT and MET. It only considers MCT amongst the $K$ percent of machines with the lowest expected execution times for an incoming task.

\subsection{Batch-Mode Mapping Heuristics for Heterogeneous Systems}
\label{subsec:baseline}
\begin{figure}[ht]%
\centering
\includegraphics[width=0.8\textwidth]{figures/C3/mapper_batch.pdf}
    \label{fig:BatchSchedule}
    \caption{Batch-mode resource allocation operates on batches of tasks upon task completion (and task arrival when machines queues are not full).}    
\end{figure}


\paragraph{MinCompletion-MinCompletion (MM)}
This heuristic has been extensively used in the literature~\cite{he2003qos,pedemonte2016accelerating,ezzatti2013efficient, salehi2016stochastic}. In the first phase of the heuristic, the virtual queue is traversed, and for each task in that queue, the machine with the minimum expected completion time is found, and a pair is made. In the second phase, for each machine with a free slot, the provisional mapping pairs are examined to find the machine-task pair with the minimum completion time, and the assignment is made to the machine queues. The process repeats itself until all machine queues are full, or until the batch queue is exhausted.

\paragraph{MinCompletion-Soonest Deadline (MSD)}
Phase one is as in MM. Phase two selects the tasks for each machine with the soonest deadline. In the event of a tie, the task with the minimum expected completion time is selected. As with MM, after each machine with an available queue slot receives a task from the provisional mapping in phase two, the process is repeated until either the virtual machine queues are full, or the unmapped task queue is empty.

\paragraph{MinCompletion-MaxUrgency (MMU)}
Urgency of task $i$ on machine $j$ is defined as $U_{ij}={1}/{(\delta_i-\mathbb{E}[C_{ij}])}$, where $\delta_i$ is the deadline of task $i$, $\mathbb{E}[C_{ij}]$ is the expected completion time of task $i$ on machine $j$. 

Phase one of MMU is the same as MM. Using the urgency equation, phase two selects the task-machine pair that has the greatest urgency, and adds that mapping to the virtual queue. The process is repeated until either the batch queue is empty, or until the virtual machine queues are full.

\paragraph{Max Ontime Completions (MOC)}
The MOC heuristic was developed in~\cite{salehi2016stochastic}. It uses the PET matrix to calculate robustness of task-machine mappings. The first mapping phase finds, for each task, the machine offering the highest robustness value. The culling phase clears the virtual queue of any tasks that fail to meet a pre-defined ($30\%$) robustness threshold. The last phase finds the three virtual mappings with the highest robustness and permutes them to find the task-machine pair that maximizes the overall robustness and maps it to that machine's virtual queue. %PAM, in contrast, chooses the pair with the minimum completion time. 
The process repeats until either all tasks in the batch queue are mapped or dropped, or until the virtual machine queues are full. 


\subsection{Mapping Heuristics for Homogeneous Systems}

\paragraph{First Come First Served - Round Robin (FCFS-RR)}~
In FCFS-RR, a task is selected in first come first serve manner and is assigned to the first available machine in a round robin manner, from Machine 0 to Machine 


\paragraph{Earliest Deadline First (EDF)}~
EDF is functionally similar to MSD heuristic for HC systems. The first phase finds the machine with the least expected completion time. Then, the second phase sorts the arrival queue in an ascending order based on tasks' deadlines. Next, the task in the head of the arrival queue is assigned to the machine with minimum expected completion time. This process is repeated until all task are mapped or the machine queues are full.

\paragraph{Shortest Job First (SJF)}~
SJF is functionally similar to MM heuristic for HC systems. The first phase finds the machine with the least expected completion time. Then, the second phase sorts the arrival queue in an ascending order based on tasks' expected execution time. Next, the task in the head of the arrival queue is assigned to the machine with minimum expected completion time. This process is repeated until all task are mapped or the machine queues are full.


%%%%%%%%%%%%%%%%%%%%
\section{Video Stream Processing}

Video streams, either in form of on-demand streaming or live streaming, usually have to be processed before sending to the viewer. The conversion processing to fit characteristics of clients' devices~\cite{CVSS,vlsc} can be called transcoding. Transcoding can encompass operations such as \emph{bit rate adjustment, spatial resolution reduction, temporal resolution (aka frame rate) reduction, and video compression standard (codec) conversion}. Transcoding can be either performed offline or in an online (\ie on-demand) manner for videos that are rarely accessed~\cite{CVSSJournal}.  However, in the case of live video streaming, it is compulsory to transcode videos in an on-demand manner because they are not available for offline processing~\cite{vlsc}. While our video stream processing platform focus on video transcoding operations, it can also handle more general processing on the video stream as well. We believe a more personalized video processing (such as on-demand customizable video and audio censorship) can become more common in the future. 


A video stream %, as shown in \ref{fig:2}
 is composed of several sequences. Each sequence itself is composed of multiple \emph{Group Of Pictures} (GOPs) with sequence header at the beginning. Each GOP contains series of frames that begin with $I$ (intra) frame, followed by a number of $P$ (predicted) frames or $B$ (bi-directional predicted) frames. In practice, each GOP is considered as a video streaming processing request with an individual deadline \cite{jokhio2011analysis,matin_paper}. Deadline violation of any request reduces QoS of the viewer. %In this study, serverless functions are modelled after some kind of video processing task.


For workload arrival patterns,
Baccour \etal~\cite{facebookvideolive18} collects and analyzes the number of lives, viewer, location, and other metadata of more than 1,500,000 live video streaming on Facebook during June and July 2018. They found the number of video streams to follow two peaks distribution daily. The difference in workload between each day of the week is small. Therefore, to accurately replicate the arrival pattern, our workload that emulates video streaming requests are generated as the series of valleys, which include a high load period and low load periods.


\subsection{Cloud-Based Video Transcoding for Video On Demand (VOD)}
\vspace{1px}
TO BE WRITTEN (from paper of Chapter~\ref{section:platform})


\subsection{Cloud-Based Video Transcoding for Live Streaming}
\vspace{1px}
TO BE WRITTEN (from paper of Chapter~\ref{section:platform})


\section{Cloud-based Video Streaming Engine (CVSE)}
\label{sec:CVSEbg}
While storing multiple versions of the same video to serve different needs is a conventional practice, Cloud-based Video Streaming Engine (CVSE) enables on-demand (\ie lazy) transcoding of video streams~\cite{CVSSJournal}. This is particularly useful for video versions that are rarely accessed. In fact, it has been proven that video streams have long-tail access pattern~\cite{darwich16} where most of video streams are rarely accessed and only a few percentage of videos are popular (hot)~\cite{miranda}. For instance, in the case of YouTube, it has been reported that only 5\% of videos are frequently accessed and the rest are rarely accessed~\cite{gill2007youtube}. This lazy on-demand processing approach enables a wider variety of video customization than what currently offered by a pre-transcoding system.
%On top of various devices dependent specification, we also expect the user requirements to be more vary in the future. For example, a user might need the audio translation or subtitle or auto censorship to screen out unwanted graphics.

\begin{figure}
\centering
    \includegraphics[width=0.5\textwidth]{figures/C4/CVSEArch3.pdf}
    \caption{Overview of Cloud-based Video Streaming Engine (CVSE) that is used for on-demand processing of video streams.}
    \label{fig:CVSE}
  \end{figure}
In the CVSE architecture, as shown in Figure~\ref{fig:CVSE}, the Splitter dispatches GOPs of the requested video stream. A GOP processing request includes the operation required along with the corresponding parameters bound to that request. Each arriving request is assigned an individual deadline and a priority by the Admission Control component. Then, the Admission Control sends the request to the shared batch queue where the request waits to be assigned by the Scheduler to one of multiple processing unit's queue. Scheduler's batch queue is managed based on a certain scheduling policy, such as FCFS (First-Come-First-Serve), Earliest-Deadline-First (EDF), Max-Urgency-First and Highest-Priority-First~\cite{matin_paper}. Most of scheduling policies are reliant on the Time Estimator component that is aware of the expected execution time of each request type (\ie different transcoding operation) on each Transcoding VMs. Such estimation can be obtained based on historic execution time information of different transcoding operations~\cite{CVSS}. 

Once a request is on a processing unit's execution queue, its operational function and required data (such as the video segment itself) is fetched to that VM and finally the request gets executed (transcoded). Video Merger component is in charge of merging processed GOPs and transfer them to the viewer. Video Merger considers an output window for each video stream to keep track of processed GOPs. The GOPs that are missing (\eg because of a failure) are requested to be resubmitted by the Admission Control component. GOPs of the videos that are getting popular are recognized by the Caching component of CVSE and are stored to enable caching-based computational reuse.


%\section{Bayesian Statistics for Resource Allocation}
